Agent Skill Evaluation and Evolution: Frameworks and Benchmarks

The growth of agent skills has transformed how agentic systems are built, evaluated, and deployed. As skill libraries continue to scale, rigorous evaluation becomes critical to ensuring their utility, quality, and safety in real-world applications. Consequently, the field is undergoing an emerging paradigm shift from isolated skill creation to automated, evaluation-driven skill evolution. In this survey, we systematically examine the landscape of skill evolution and evaluation beyond foundational skill creation. We categorize evolution into four distinct paradigms, spanning execution feedback, trajectory distillation, compression, and reinforcement learning, showing how each element contributes to improving skill utility and reliability. We also provide an analysis of six skill-centric benchmark categories, identifying structural gaps in benchmark coverage, trade-offs, and metric richness to advance skill research. Finally, we identify open directions for building skill ecosystems that are generalizable, efficient, and verifiably safe. The project URL is https://github.com/Cassie07/AgentSkill_Survey

==> Figures/agent_skills_lifecycle_figure.tex <==
% Agent Skill Lifecycle — Summary Figure
% Compile with: pdflatex or lualatex (requires TikZ, xcolor)

% ── Color palette ──────────────────────────────────────────────
\definecolor{clrPurpleLight}{HTML}{EEEDFE}
\definecolor{clrPurpleMid}  {HTML}{534AB7}
\definecolor{clrPurpleDark} {HTML}{3C3489}

\definecolor{clrTealLight}  {HTML}{E1F5EE}
\definecolor{clrTealMid}    {HTML}{0F6E56}
\definecolor{clrTealDark}   {HTML}{085041}

\definecolor{clrBlueLight}  {HTML}{E6F1FB}
\definecolor{clrBlueMid}    {HTML}{185FA5}
\definecolor{clrBlueDark}   {HTML}{0C447C}

\definecolor{clrAmberLight} {HTML}{FAEEDA}
\definecolor{clrAmberMid}   {HTML}{854F0B}
\definecolor{clrAmberDark}  {HTML}{633806}

\definecolor{clrCoralLight} {HTML}{FAECE7}
\definecolor{clrCoralMid}   {HTML}{993C1D}
\definecolor{clrCoralDark}  {HTML}{712B13}

\definecolor{clrGrayLight}  {HTML}{F1EFE8}
\definecolor{clrGrayMid}    {HTML}{5F5E5A}
\definecolor{clrGrayDark}   {HTML}{444441}

% ── TikZ styles ────────────────────────────────────────────────
\tikzset{
  skillbox/.style={
    rectangle, rounded corners=6pt,
    minimum width=#1, minimum height=1.0cm,
    inner sep=5pt, align=center,
    font=\footnotesize\sffamily,
    draw, line width=0.4pt,
  },
  skillbox/.default=3.5cm,
  labelbox/.style={
    skillbox=2.5cm,
    minimum height=0.85cm,
    font=\footnotesize\sffamily\bfseries,
  },
  detailbox/.style={
    skillbox=2.5cm,
    minimum height=0.85cm,
    font=\scriptsize\sffamily,
  },
  sectionbox/.style={
    skillbox=2.5cm,
    minimum height=1.2cm,
    font=\small\sffamily\bfseries,
  },
  myarrow/.style={
    -{Stealth[length=4pt,width=3pt]},
    line width=0.6pt,
    color=clrGrayMid,
  },
  childarrow/.style={
    -{Stealth[length=3pt,width=2.5pt]},
    line width=0.4pt,
    color=clrGrayMid,
  },
  detailarrow/.style={
    -{Stealth[length=3pt,width=2.5pt]},
    line width=0.4pt,
    color=clrGrayMid,
  },
  col/purple/.style={fill=clrPurpleLight, draw=clrPurpleMid, text=clrPurpleDark},
  col/teal/.style  ={fill=clrTealLight,   draw=clrTealMid,   text=clrTealDark},
  col/blue/.style  ={fill=clrBlueLight,   draw=clrBlueMid,   text=clrBlueDark},
  col/amber/.style ={fill=clrAmberLight,  draw=clrAmberMid,  text=clrAmberDark},
  col/coral/.style ={fill=clrCoralLight,  draw=clrCoralMid,  text=clrCoralDark},
  col/gray/.style  ={fill=clrGrayLight,   draw=clrGrayMid,   text=clrGrayDark},
}

\newcommand{\sub}[1]{{\scriptsize\color{clrGrayMid}#1}}

\begin{figure*}[t!]
\centering
\begin{tikzpicture}[
  node distance = 1cm and 1cm,
]

% ============================================================
% A–D COLUMN — fixed absolute positions
% ============================================================

% ── A. Skill creation ─────────────────────────────────
\node[sectionbox, col/teal] at (5cm, 0cm)
  (A) {\textbf{A. Skill creation}\\[1pt]\sub{§2}};

\node[labelbox, col/teal, right=0.55cm of A, yshift=0.55cm]
  (A1) {Human-written};
\node[detailbox, col/teal, right=0.3cm of A1]
  (A1d) {Domain experts, partners};
\draw[detailarrow] (A1.east) -- (A1d.west);

\node[labelbox, col/teal, below=0.2cm of A1]
  (A2) {Automated creation};
\node[detailbox, col/teal, right=0.3cm of A2]
  (A2d) {Voyager, skill-creator, SAGE, ARISE};
\draw[detailarrow] (A2.east) -- (A2d.west);

\node[labelbox, col/teal, below=0.2cm of A2]
  (A3) {Open repositories};
\node[detailbox, col/teal, right=0.3cm of A3]
  (A3d) {anthropics/skills, SkillsMP};
\draw[detailarrow] (A3.east) -- (A3d.west);

\draw[childarrow] (A.east) -- (A1.west);
\draw[childarrow] (A.east) -- (A2.west);
\draw[childarrow] (A.east) -- (A3.west);

% ── B. Skill selection ────────────────────────────────
\node[sectionbox, col/blue, below=2.3cm of A]
  (B) {\textbf{B. Skill usage}\\[1pt]\sub{§3}};

\node[labelbox, col/blue, right=0.55cm of B, yshift=0.55cm]
  (B1) {Retrieval};
\node[detailbox, col/blue, right=0.3cm of B1]
  (B1d) {SkillFlow, SkillRouter};
\draw[detailarrow] (B1.east) -- (B1d.west);

\node[labelbox, col/blue, below=0.2cm of B1]
  (B2) {Routing};
\node[detailbox, col/blue, right=0.3cm of B2]
  (B2d) {SkillOrchestra};
\draw[detailarrow] (B2.east) -- (B2d.west);


\node[labelbox, col/blue, below=0.2cm of B2]
  (B3) {Storage};
\node[detailbox, col/blue, right=0.3cm of B3]
  (B3d) {AgentSkillOS};
\draw[detailarrow] (B3.east) -- (B3d.west);


\draw[childarrow] (B.east) -- (B1.west);
\draw[childarrow] (B.east) -- (B2.west);
\draw[childarrow] (B.east) -- (B3.west);

% ── C. Skill evolution ────────────────────────────────
\node[sectionbox, col/amber, below=2.5cm of B]
  (C) {\textbf{C. Skill evolution}\\[1pt]\sub{§4}};

\node[labelbox, col/amber, right=0.55cm of C, yshift=0.80cm]
  (C1) {Execution feedback};
\node[detailbox, col/amber, right=0.3cm of C1]
  (C1d) {SkillForge, CoEvoSkills, Skills-Coach, \\Ctx2Skill, AutoSkill, SkillClaw};
\draw[detailarrow] (C1.east) -- (C1d.west);

\node[labelbox, col/amber, below=0.2cm of C1]
  (C2) {Trajectory distillation};
\node[detailbox, col/amber, right=0.3cm of C2]
  (C2d) {Trace2Skill, XSkill, Memento-Skills};
\draw[detailarrow] (C2.east) -- (C2d.west);

\node[labelbox, col/amber, below=0.2cm of C2]
  (C3) {Compression \\and Augmentation};
\node[detailbox, col/amber, right=0.3cm of C3]
  (C3d) {SkillNet, SkillX, SkillReducer, \\SkillFoundry};
\draw[detailarrow] (C3.east) -- (C3d.west);

\node[labelbox, col/amber, below=0.2cm of C3]
  (C4) {RL-driven evolution};
\node[detailbox, col/amber, right=0.3cm of C4]
  (C4d) {D2Skill, SkillRL, Skill1};
\draw[detailarrow] (C4.east) -- (C4d.west);

\draw[childarrow] (C.east) -- (C1.west);
\draw[childarrow] (C.east) -- (C2.west);
\draw[childarrow] (C.east) -- (C3.west);
\draw[childarrow] (C.east) -- (C4.west);

% ── D. Skill evaluation ───────────────────────────────
\node[sectionbox, col/gray, below=3cm of C]
  (D) {\textbf{D. Skill evaluation}\\[1pt]\sub{§5}};

\node[labelbox, col/gray, right=0.55cm of D, yshift=0.35cm]
  (D1) {Static benchmarks};
\node[detailbox, col/gray, right=0.3cm of D1]
  (D1d) {ALFWorld, SWE-bench, GAIA};
\draw[detailarrow] (D1.east) -- (D1d.west);

\node[labelbox, col/gray, below=0.2cm of D1]
  (D2) {Dynamic benchmarks};
\node[detailbox, col/gray, right=0.3cm of D2]
  (D2d) {SkillsBench, SkillTester};
\draw[detailarrow] (D2.east) -- (D2d.west);

\draw[childarrow] (D.east) -- (D1.west);
\draw[childarrow] (D.east) -- (D2.west);

% ============================================================
% TITLE — vertically centered between B and C, to the left
% ============================================================
% A=0, B≈-3.7, C≈-7.7, D≈-12.4 → midpoint of full range ≈ -6.2
% Tune this value until it sits between B and C visually
\node[sectionbox, col/purple, minimum width=3cm, minimum height=1.1cm]
  (title) at (0cm, -6.2cm) {\textbf{Agent skill lifecycle}\\[1pt]\sub{§2 - 5}};

% ── Spine: vertical chain A→B→C→D ─────────────────────────
\draw[myarrow] (A.south) -- (B.north);
\draw[myarrow] (B.south) -- (C.north);
\draw[myarrow] (C.south) -- (D.north);

% ── Title → A,B,C,D: fan-out straight arrows ──────────────
% Same style as A→A1/A2/A3 (diagonal from single point)
\draw[childarrow] (title.east) -- (A.west);
\draw[childarrow] (title.east) -- (B.west);
\draw[childarrow] (title.east) -- (C.west);
\draw[childarrow] (title.east) -- (D.west);

\end{tikzpicture}
\caption{Overview of the agent skill lifecycle covered in this survey, including A. Skill creation, B. Skill usage, C. Skill evolution, and D. Skill evaluation.}
\label{fig:agent-skill-lifecycle}
\end{figure*}

==> sections/11_revision.tex <==
% \section{Skill Evolution Strategy Comparison and Selection}
% \label{supp_skill_comparison}

% \input{tables/tab_revision_comparison}
% \input{Figures/Revision_workflow}




==> tables/detail_rebuttal.tex <==
% =====================================================================
% Qualitative comparison of skill-evolution systems (Section 3 / Sec.~2.3).
% Motivation: the 30+ surveyed systems use different base models, task
% types, and evaluation protocols, so raw "A > B" claims are not
% comparable. This table gives readers actionable, side-by-side criteria
% (base/executor model, task domain, headline reported result, and
% open-source status) rather than a single leaderboard number.
%
% Requires in preamble:
%   \usepackage{booktabs}
%   \usepackage{tabularx}
%   \usepackage{makecell}
%   \usepackage[table]{xcolor}
%   \usepackage{array}
%   \usepackage{fontawesome5}   % for \faCheck / \faTimes (optional)
%
% Reuses the category colors already defined in table_skill_evolution.tex:
%   catFeedback, catDistill, catCompAug, catRL
% If this table is compiled standalone, uncomment the four \definecolor lines.
% \definecolor{catFeedback}{RGB}{255,229,204}
% \definecolor{catDistill}{RGB}{217,234,211}
% \definecolor{catCompAug}{RGB}{207,226,243}
% \definecolor{catRL}{RGB}{230,217,243}

\newcommand{\yes}{\textcolor{green!55!black}{\faCheck}}
\newcommand{\no}{\textcolor{red!70!black}{\faTimes}}

\begin{table*}[t!]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.25}
\renewcommand{\tabularxcolumn}[1]{>{\raggedright\arraybackslash}m{#1}}
\begin{tabularx}{\textwidth}{@{}%
  >{\raggedright\arraybackslash}m{1.75cm}%
  >{\raggedright\arraybackslash}m{2.7cm}%
  >{\raggedright\arraybackslash}m{2.5cm}%
  X%
  >{\centering\arraybackslash}m{0.7cm}@{}}
\toprule
\rowcolor{black!8}\textbf{System} & \textbf{Base / executor model} & \textbf{Task domain} & \textbf{Reported headline result (as stated by authors)} & \textbf{Open src.} \\
\midrule

%% ---- Execution Feedback -------------------------------------------------
\rowcolor{catFeedback}\multicolumn{5}{@{}l}{\textbf{\faSync~Execution Feedback}}\\
SkillForge~{\footnotesize\cite{liu2026skillforge}}
  & Qwen3-Max (internal)
  & Cloud technical support
  & Self-evolution loop progressively improves skill quality on 5 cloud-support scenarios (1{,}883 tickets / 3{,}737 tasks); consistency with expert references
  & \yes \\
CoEvoSkills~{\footnotesize\cite{zhang2026coevoskills}}
  & Claude Opus 4.6 (+ Claude Code, Codex)
  & SkillsBench (11 pro.\ domains)
  & 71.1\% pass rate on SkillsBench ($+40.5$pp over no-skill); transfers to 6 further LLMs
  & \yes \\
Skills-Coach~{\footnotesize\cite{tian2026skills}}
  & Not tied to one backbone (training-free GRPO)
  & Skill-X (48 skills)
  & Consistent gains across skill categories; competitive results in minutes vs.\ hours
  & \yes \\
Ctx2Skill~{\footnotesize\cite{si2026context}}
  & GPT-4.1 / GPT-5.1 / GPT-5.2
  & CL-bench (context learning)
  & $+3.2$ to $+5.5$pp solving rate over no-skill; weaker model + skills beats stronger model without
  & \yes \\
AutoSkill~{\footnotesize\cite{yang2026autoskill}}
  & Model-agnostic plugin layer
  & Dialogue / interaction traces (StuLife-style ELL)
  & Learned skills improve perceived quality \& factual reliability at modest added latency
  & \yes \\
SkillClaw~{\footnotesize\cite{ma2026skillclaw}}
  & Qwen3-Max
  & WildClawBench (real-world assistant)
  & Improves Qwen3-Max under limited group interaction ``not by using a bigger model''
  & \yes \\
EmbodiSkill~{\footnotesize\cite{ju2026embodiskill}}
  & Qwen3.5-27B / Qwen3-VL-32B (frozen executor)
  & ALFWorld, EmbodiedBench
  & 93.28\% ALFWorld success; $+31.58$pp over GPT-5.2 direct agent
  & \no \\
\midrule

%% ---- Trajectory Distillation --------------------------------------------
\rowcolor{catDistill}\multicolumn{5}{@{}l}{\textbf{\faRoute~Trajectory Distillation}}\\
SPARK~{\footnotesize\cite{zhou2026evidence}}
  & Teacher: Claude Opus 4.6; student: GPT-5.4-mini / DeepSeek
  & SkillsBench (86 runnable tasks)
  & Beats no-skill and human-written skills on students; up to $1000\times$ cheaper than teacher (e.g.\ DeepSeek 9.1\%$\rightarrow$42.4\%)
  & \yes \\
Trace2Skill~{\footnotesize\cite{ni2026trace2skill}}
  & Qwen3.5-35B (evolve) $\rightarrow$ 122B (transfer)
  & Spreadsheet, math, VisionQA, WikiTQ
  & Up to $+57.65$pp on WikiTableQuestions (35B-evolved skills applied to 122B agent)
  & \yes \\
Memento-Skills~{\footnotesize\cite{zhou2026memento}}
  & Not fixed (external skill memory; no weight updates)
  & GAIA, HLE
  & $+26.2\%$ / $+116.2\%$ relative overall accuracy on GAIA / HLE
  & \yes \\
XSkill~{\footnotesize\cite{jiang2026xskill}}
  & 4 backbone models (multimodal)
  & VisualToolBench, TIR-Bench, MMSearch-Plus, AgentVista, MMBrowseComp
  & Avg.\ $+2.58$ to $+6.71$ pts over strong baselines; zero-shot transfer (ICML~2026)
  & \yes \\
\midrule

%% ---- Compression & Augmentation ----------------------------------------
\rowcolor{catCompAug}\multicolumn{5}{@{}l}{\textbf{\faCompress~Compression \& Augmentation}}\\
SkillNet~{\footnotesize\cite{liang2026skillnet}}
  & Multiple backbones
  & ALFWorld, WebShop, ScienceWorld
  & $\sim+40\%$ avg reward, $-30\%$ execution steps across backbones
  & \yes \\
SkillX~{\footnotesize\cite{wang2026skillx}}
  & GLM-4.6 (build) $\rightarrow$ Qwen3-32B / Kimi-K2 / GLM-4.6 (deploy)
  & AppWorld, BFCL-v3, $\tau^2$-Bench
  & $\sim$10-point improvement on several benchmarks when plugged into weaker agents
  & \yes \\
SkillReducer~{\footnotesize\cite{gao2026skillreducer}}
  & 5 models / 4 families
  & SkillsBench + 600 curated skills (coding)
  & 48\% description / 39\% body token reduction with $+2.8\%$ functional quality; retention 0.965
  & --- \\
SkillFoundry~{\footnotesize\cite{shen2026skillfoundry}}
  & Coding agent (+ Biomni for genomics)
  & MoSciBench + genomics workflows
  & 71.1\% of mined skills novel; improves 5/6 MoSciBench datasets \& 2 genomics tasks
  & \yes \\
\midrule

%% ---- Reinforcement Learning ---------------------------------------------
\rowcolor{catRL}\multicolumn{5}{@{}l}{\textbf{\faTrophy~Reinforcement Learning}}\\
D2Skill~{\footnotesize\cite{tu2026dynamic}}
  & Qwen2.5-7B-Instruct / Qwen3-4B-Instruct
  & ALFWorld, WebShop, search-aug.\ QA
  & 90.6 ALFWorld / 84.4 WebShop (7B); ALFWorld 53.9$\rightarrow$72.7 over GRPO (4B)
  & --- \\
SkillRL~{\footnotesize\cite{xia2026skillrl}}
  & Qwen2.5-7B-Instruct (+ o3 teacher)
  & ALFWorld, WebShop, 7 search-aug.\ QA
  & 89.9\% ALFWorld / 72.7\% WebShop; $+15.3\%$ over memory-augmented RL; $+12.3$pp over GRPO on ALFWorld
  & --- \\
SkillOS~{\footnotesize\cite{ouyang2026skillos}}
  & Frozen executor + trainable curator (multiple backbones)
  & Multi-turn agentic + single-turn reasoning
  & Outperforms memory-free \& memory-based baselines; curator generalizes across executor backbones
  & --- \\
Skill1~{\footnotesize\cite{shi2026skill1}}
  & Single RL policy (co-evolved)
  & ALFWorld, WebShop
  & Outperforms prior skill-based \& RL baselines; selection precision 0.95 by step~20
  & \yes \\
\bottomrule
\end{tabularx}
\caption{Qualitative comparison of the skill-evolution systems surveyed in \autoref{sec:2.3}.
Because these systems are evaluated on different base models, task suites, and protocols, their reported numbers are \emph{not} directly comparable; a single leaderboard would conflate skill quality with base-model capability.
We therefore list, for each system, its base/executor model, task domain, the headline result exactly as reported by its authors, and whether code is publicly released, so readers can apply their own comparison criteria when selecting a method.
Categories are color-coded as in \autoref{tab:evolution_categories}:
\catbox{catFeedback}~Execution Feedback,\;
\catbox{catDistill}~Trajectory Distillation,\;
\catbox{catCompAug}~Compression \& Augmentation,\;
\catbox{catRL}~Reinforcement Learning.
Reported results use each paper's own metric and baseline and should be read within that paper's setting only.
Open src.: \yes~= code released; \no~= no public code found; ---~= not clearly stated at time of writing.}
\label{tab:evolution_comparison}
\end{table*}
